Query-Efficient Correlation Clustering with Noisy Oracle

We study a general clustering setting in which we have $n$ elements to be clustered, and we aim to perform as few queries as possible to an oracle that returns a noisy sample of the weighted similarity between two elements. Our setting encompasses many application domains in which the similarity function is costly to compute and inherently noisy. We introduce two novel formulations of online learning problems rooted in the paradigm of Pure Exploration in Combinatorial Multi-Armed Bandits (PE-CMAB): fixed confidence and fixed budget settings. For both settings, we design algorithms that combine a sampling strategy with a classic approximation algorithm for correlation clustering and study their theoretical guarantees. Our results are the first examples of polynomial-time algorithms that work for the case of PE-CMAB in which the underlying offline optimization problem is NP-hard.

==> heuristic.tex <==
As we will see in Section~\ref{sec:experiments}, algorithm $\ouralg$, while provably optimal up to constant factors, sometimes returns solutions with poor recall of positive edges
when the query budget is low. Intuitively, the reason is that, while picking a random pivot works in expectation, sometimes a low-degree pivot is chosen and all $|R|-1$ queries are spent querying
its neighbors, which may not be worth the effort for a small cluster when the query budget is tight. To entice the algorithm to choose higher-degree vertices (which would also improve the recall), we propose to bias it so that pivots are chosen with probability
proportional to their positive degree in the subgraph induced by $R$. The conclusion of Lemma~\ref{lem:indep} remains unaltered in this case, but whether this change preserves the
approximation guarantees from ~\cite{balls} on which we rely is unclear.
In practice, this heuristic modification consistently
improves the recall on all the tests we performed, as well as the total number of disagreements in most cases.

\mycomment{
We cannot afford to compute the degree of each vertex with a small number of queries, but
the following scheme is easily seen to choose each vertex $u \in R$ with probability $(1 + d_u) / (|R| + 2E)$, where $d_u$ is the degree of $u$ in the subgraph $G[R]$ induced by $R$ and $E$ is the
total number of edges in $G[R]$:
\begin{enumerate}
    \item Pick random pairs of vertices $(u, v) \in R \times R$ until $u = v$ or an edge $(u, v) \in E$ is found;
    \item Select the first  endpoint $u$ of this edge as a pivot.
\end{enumerate}
The reason we sample with probability proportional to $1+d_u$ instead of $d_u$ is to avoid infinite loops when $G[R]$ contains no edges.
}
We cannot afford to compute the degree of each vertex with a small number of queries, but
the following scheme is easily seen to choose each vertex $u \in R$ with probability $d_u / (2E)$, where $d_u$ is the degree of $u$ in the subgraph $G[R]$ induced by $R$, and $E>0$ is the
total number of edges in $G[R]$:
\begin{enumerate}
    \item Pick random pairs of vertices to query $(u, v) \in R \times R$ until an edge $(u, v) \in E$ is found;
    \item Select the first endpoint $u$ of this edge as a pivot.
\end{enumerate}
When $E = 0$, this procedure will simply run out of queries to make.

%Indeed, $u$ is chosen uniformly at random from $R$, and the probability that another randomly chosen vertex is a neighbor is exactly $d_u/(|R| - 1)$, where $d_u$ denotes the degree of $u$. It follows that this scheme

Pseudocode for $\ourheur$ is shown below.
\begin{algorithm}\label{alg:our_heur}
\begin{algorithmic}[0]
\Require $G = (V, E)$; query budget $Q$
\State $R \gets V$ \Comment Unclustered vertices so far
\While {$|R| > 1 \wedge Q \ge |R| - 1$}
\State Pick a pair $(u, v)$ from $R \times R$ uniformly at random.
\State \If { $u \neq v$ }
\State Query $(u, v)$
\State $Q \gets Q - 1$
%\State \If {$u = v$ \textbf{or} $(u, v) \in E$ }
\State \If { $(u, v) \in E$ }
\State Query all pairs $(v, w)$ for $w \in R\setminus \{u, v\}$ 
\State \; to determine $\Gamma_G^+(v) \cap R$.
\State $Q \gets Q - |R| + 2$.
\State Output cluster $C = \{v\} \cup \Gamma_G^+(v) \cap R$.
\State $R \gets V \setminus C$
\EndIf
\EndIf
\EndWhile
\State Output a separate singleton cluster for each remaining $v \in R$.
\caption{\ourheur}
\end{algorithmic}
\end{algorithm}

